Read Disturb Errors in MLC NAND Flash Memory

This paper summarizes our work on experimentally characterizing, mitigating, and recovering read disturb errors in multi-level cell (MLC) NAND flash memory, which was published in DSN 2015, and examines the work's significance and future potential. NAND flash memory reliability continues to degrade as the memory is scaled down and more bits are programmed per cell. A key contributor to this reduced reliability is read disturb, where a read to one row of cells impacts the threshold voltages of unread flash cells in different rows of the same block. For the first time in open literature, this work experimentally characterizes read disturb errors on state-of-the-art 2Y-nm (i.e., 20-24 nm) MLC NAND flash memory chips. Our findings (1) correlate the magnitude of threshold voltage shifts with read operation counts, (2) demonstrate how program/erase cycle count and retention age affect the read-disturb-induced error rate, and (3) identify that lowering pass-through voltage levels reduces the impact of read disturb and extend flash lifetime. Particularly, we find that the probability of read disturb errors increases with both higher wear-out and higher pass-through voltage levels. We leverage these findings to develop two new techniques. The first technique mitigates read disturb errors by dynamically tuning the pass-through voltage on a per-block basis. Using real workload traces, our evaluations show that this technique increases flash memory endurance by an average of 21%. The second technique recovers from previously-uncorrectable flash errors by identifying and probabilistically correcting cells susceptible to read disturb errors. Our evaluations show that this recovery technique reduces the raw bit error rate by 36%.

==> Makefile <==
################################################################################
# Custom Rules
################################################################################

SRC  = $(shell egrep -l '^[^%]*\\begin\{document\}' *.tex)
TRG  = $(SRC:%.tex=%.pdf)

all: $(TRG)
.PHONY: $(TRG) clean rolling

################################################################################
# Latexmk Rules
################################################################################
# -pdf: Generate pdf version of document using pdflatex.
#
# -bibtex: When the source file uses bbl files for bibliography, run bibtex or
#  biber as needed to regenerate the bbl files.
#
#  -C: Clean up (remove) all regeneratable files generated by latex and bibtex
#  or biber.
################################################################################

rolling: $(SRC)
	latexmk -pvc -pdf -bibtex -interaction=nonstopmode $(SRC)

$(TRG): $(SRC) *.tex
	latexmk -pdf -bibtex $(SRC)

clean:
	latexmk -c -bibtex


